Measurement-Adaptive Sparse Image Sampling and Recovery

This paper presents an adaptive and intelligent sparse model for digital image sampling and recovery. In the proposed sampler, we adaptively determine the number of required samples for retrieving image based on space-frequency-gradient information content of image patches. By leveraging texture in space, sparsity locations in DCT domain, and directional decomposition of gradients, the sampler structure consists of a combination of uniform, random, and nonuniform sampling strategies. For reconstruction, we model the recovery problem as a two-state cellular automaton to iteratively restore image with scalable windows from generation to generation. We demonstrate the recovery algorithm quickly converges after a few generations for an image with arbitrary degree of texture. For a given number of measurements, extensive experiments on standard image-sets, infra-red, and mega-pixel range imaging devices show that the proposed measurement matrix considerably increases the overall recovery performance, or equivalently decreases the number of sampled pixels for a specific recovery quality compared to random sampling matrix and Gaussian linear combinations employed by the state-of-the-art compressive sensing methods. In practice, the proposed measurement-adaptive sampling/recovery framework includes various applications from intelligent compressive imaging-based acquisition devices to computer vision and graphics, and image processing technology. Simulation codes are available online for reproduction purposes.

==> mathabx.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathabx.tex. Version: May 18, 2005.
% Author: Anthony PHAN.
% matches the ``mathabx'' family.
% plain-TeX input file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ifx\mathabxversion\undefined\else\endinput\fi
\def\mathabxversion{January 28, 2004}%
%
\catcode`@=11
%
% proofing?
%

\ifx\proofmode\undefined
	\def\symbol@message#1{\relax}%
	\def\symbol@mark#1#2{\relax}%
	\def\check@definition#1{\relax}%
	\def\mathabx@undefine#1{\let#1=\undefined}%
	\def\mathabx@aliases#1#2{\@mathabx@aliases#1#2?\@end}
	\def\@mathabx@aliases#1#2#3\@end{\ifx#2?\else
		\let#2=#1\@mathabx@aliases#1#3\@end\fi}%
\else
	\def\symbol@message#1{\vskip\z@ plus\baselineskip
		\penalty-250\vskip\z@ plus-\baselineskip
		\medbreak{\noindent\bf #1}%
		\nobreak\smallskip\noindent\ignorespaces}%
	\def\symbolsp@cing#1{\ifcase\number#1 ord\or op%
		\or bin\or rel\or open\or close\or punct%
		\or var\else other\fi}%
	\def\symbol@mark#1#2{\allowbreak
		\hbox to 0.05\hsize{$#1$\hss}%
		\hbox to 0.05\hsize{\unhbox0\hss}%
		\hbox to 0.4001\hsize{{\tt\string#1}%
		$^{\rm\symbolsp@cing{#2}}$\hfil}%
		\ignorespaces}%
	\def\check@definition#1{\ifx#1\undefined
		\setbox0\hbox{}%
		\else\setbox0=\hbox{$#1\relax$}\fi}%
	\def\mathabx@undefine#1{}%
	\def\mathabx@aliases#1#2{\setbox0=\lastbox
		\@mathabx@aliases#1#2?\@end
		\ifdim\wd0>0.4\hsize\hbox to 0.9001\hsize{\unhbox0\hfill}%
		\else\hbox to 0.4001\hsize{\unhbox0\hfill}\fi}%
	\def\@mathabx@aliases#1#2#3\@end{\ifx#2?\else
		\let#2=#1%
		\setbox0=\hbox{\unhbox0, \tt\string#2}%
		\@mathabx@aliases#1#3\@end\fi}%
\fi
%
% Symbols declarations: \LaTeX-like commands
%
\def\hexnumber@#1{\ifcase\number#1 0\or 1\or 2\or 3\or 4%
	\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\else F\fi}%
\def\hexnumber@@#1{{\count0=#1
	\count1=#1
	\divide\count0 by 16
	\hexnumber@\count0
	\multiply\count0 by 16
	\advance\count1 by -\count0
	\hexnumber@\count1}}%
%
\def\DeclareMathSymbol#1#2#3#4{\check@definition{#1}%
	\count255=#2\multiply\count255 by 16
	\advance\count255 by \csname#3fam\endcsname
	\multiply\count255 by 256\advance\count255 by #4
	\ifcat\noexpand#1\relax\mathchardef#1=\count255%
	\else\expandafter
		\mathcode\expandafter`\csname#1\endcsname=\count255%
	\fi\symbol@mark{#1}{#2}}%
%
\def\gobble@quotes#1{\ifx#1"\else#1\fi}%
%
\def\@DeclareMathDelimiter#1#2#3#4#5#6{%
	\edef#1{\noexpand\delimiter\noexpand"\gobble@quotes#2%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4%
	\expandafter\hexnumber@\csname#5fam\endcsname\gobble@quotes#6 }%
	\symbol@mark{#1}{#2}}%
%
\def\@xDeclareMathDelimiter#1#2#3#4#5{%
	\count255=\csname#2fam\endcsname
	\multiply\count255 by 256\advance\count255 by #3
	\multiply\count255 by 16
	\advance\count255 by \csname#4fam\endcsname
	\multiply\count255 by 256\advance\count255 by #5
	\expandafter\delcode\expandafter`\csname#1\endcsname=\count255
	\symbol@mark{#1}{8}}%
%
\def\DeclareMathDelimiter#1{\check@definition{#1}%
	\ifcat\noexpand#1\relax
	\def\Large@stuff{\noexpand\delimiter}%
	\expandafter\@DeclareMathDelimiter
	\else\expandafter\@xDeclareMathDelimiter\fi#1}%
%
\def\DeclareMathRadical#1#2#3#4#5{%\check@definition{#1}%
	\edef#1{\noexpand\radical\noexpand"%
	\expandafter\hexnumber@\csname#2fam\endcsname\gobble@quotes#3%
	\expandafter\hexnumber@\csname#4fam\endcsname\gobble@quotes#5 }%
	\symbol@mark{#1{}}{8}}%
%
\def\DeclareMathAccent#1#2#3#4{%\check@definition{#1}%
        \edef#1{\noexpand\mathaccent\noexpand"%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4 }%
	\symbol@mark{#1{}}{8}}%
%
% loading math fonts
%
\font\twelvematha=matha10 at 12pt
\font\tenmatha=matha10  \font\ninematha=matha9
\font\eightmatha=matha8 \font\sevenmatha=matha7
\font\sixmatha=matha6   \font\fivematha=matha5
\newfam\mathafam
\font\twelvemathb=mathb10 at 12pt
\font\tenmathb=mathb10  \font\ninemathb=mathb9
\font\eightmathb=mathb8 \font\sevenmathb=mathb7
\font\sixmathb=mathb6   \font\fivemathb=mathb5
\newfam\mathbfam
\font\tenmathx=mathx10
\newfam\mathxfam
%\chardef\mathxfam=4
%\let\tenex=\tenmathx
%
% Initialization
% (make changes in your own file if you want different sizes)
%
\textfont\mathafam=\tenmatha  \scriptfont\mathafam=\sevenmatha
\scriptscriptfont\mathafam=\fivematha
\textfont\mathbfam=\tenmathb  \scriptfont\mathbfam=\sevenmathb
\scriptscriptfont\mathbfam=\fivemathb
\textfont\mathxfam=\tenmathx  \scriptfont\mathxfam=\tenmathx
\scriptscriptfont\mathxfam=\tenmathx
%\def\dagesh#1{{\fam\mathbfam#1}}%
\def\mathafont{\fam\mathafam\tenmatha}%
\def\mathbfont{\fam\mathbfam\tenmathb}%
\let\mathabx@matha=\relax
\let\mathabx@mathb=\relax
\let\mathabx@mathx=\relax
\let\end@mathabx=\relax
\input mathabx.dcl
\catcode`@=12
\let\proofmode=\undefined
\endinput



